Specification-Guided Critical Scenario Identification for Automated Driving

To test automated driving systems, we present a case study for finding critical scenarios in driving environments guided by formal specifications. To that aim, we devise a framework for critical scenario identification, which we base on open-source libraries that combine scenario specification, testing, formal methods, and optimization.

==> leftovers.tex <==
\newpage
\appendix

\section{Signal Temporal Logic}

We start with some background definitions.Let $\esses = \{s_1,\hdots,s_n\}$ be a set of real-valued variables. The time domain $\T$  is of the form $[0,d]\subset \R$.
A \emph{signal} $w$ is a function $\T \to \R^n$, which we also see as a vector of real-valued signals $w_i : \T \to \R$ associated to variables $s_i$ for $i=1,\hdots,n$.
Given two signals $u : \T \to \R^l$ and $v : \T \to \R^m$, we define their parallel composition $u \| v : \T \to \R^{l+m}$ in the expected way.
Given a signal $w : \T \to \R^n$ and variables $\ares \subseteq \esses$ with $\ares = \{ s_{i_1},\hdots,s_{i_m} \}$ for some $1 \le i_1 <\hdots <i_m \le n$, we define the projection of $w$ onto $R$ as follows: $w_\ares = w_{i_1}\| \hdots \| w_{i_m}$.

\subsubsection{Syntax}

Let $\tees$ be a set of terms of the form $f(\ares)$ where $\ares \subseteq \esses$ are subsets of variables and $f : \R^{|\ares|} \to \R$ are interpreted functions.
The syntax of STL is given by the grammar
\begin{align*}
\f ::= \true \mid f(\ares) > 0 \mid \lnot \f \mid \f_1 \lor \f_2 \mid \f_1 \until_I \f_2 \,,
\end{align*}
where $f(R)$ are terms in $\tees$ and $I$ are real intervals with bounds in $\mathbb Q_{\ge 0} \cup \{\infty\}$.
As customary we use the shorthands $\eventually_I \f \equiv \true \until_I \f$ for \emph{eventually} and $\always_I \f \equiv \lnot \eventually_I \lnot \f$ for \emph{always}.
The timing interval $I$ may be omitted when $I=[0,\infty)$ or $I=(0,\infty)$.

We now define {\em interface-aware signal temporal logic} (IA-STL), by augmenting STL with input/output declarations.
Formally, an IA-STL specification is a tuple $(\exes, \wyes, \f)$ such that $\exes \cap \wyes = \emptyset$, where 
\begin{itemize}
    \item $\f$ is an STL formula over variables in $\esses$;
    \item $\exes \subseteq \esses$ is the set of the {\em input} variables;
    \item $\wyes \subseteq \esses$ is the set of the {\em output} variables.
\end{itemize}
We remark that while desirable, we do not require the set of signals to be partitioned into input and outputs, in that we allow for signals in $\esses \setminus (\exes \cup \wyes)$ that are neither input nor output. This may be relevant for internal state signals whose role is not clearly defined. This also ensures backward compatibility and in general makes IA-STL a conservative extension of STL.


\subsubsection{Robustness Semantics}

We introduce a notion of robustness specialized according to two subsets of variables $\exes,\wyes \subseteq \esses$ such that $\exes \cap \wyes = \emptyset$.
Let $\f$ be an STL formula and $w$ a signal trace.
We define the $\exes$-robustness relative to $\wyes$, denoted $\rho_\exes^\wyes(\f,w,t)$ by induction as follows:
%
\begin{align*}
\rho_\exes^\wyes(\true, w, t) &= +\infty \\
\rho_\exes^\wyes(f(\ares) > 0, w, t) &= 
	\begin{cases}
		0 &\text{if } \ares \nsubseteq \exes\cup \wyes \\
		f(w_\ares[t]) &\text{else if } \ares \nsubseteq \wyes \\
		\sign(f(w_\ares[t])) \cdot \infty &\text{otherwise}
	\end{cases}\\
\rho_\exes^\wyes(\lnot \f, w, t) &= -\rho_\exes^\wyes(\f, w, t) \\
\rho_\exes^\wyes(\f_1 \lor \f_2, w, t) &= \max \left\{ \rho_\exes^\wyes(\f_1, w, t), \rho_\exes^\wyes(\f_2, w, t) \right\} \\
\rho_\exes^\wyes(\f_1 \until_I \f_2, w, t) &= \sup_{t' \in t \oplus I} \min\left\{\begin{array}{c} \rho_\exes^\wyes(\f_2, w, t') , \\ \inf_{t'' \in (t,t')} \rho_\exes^\wyes(\f_1, w, t'') \end{array}\right\},
\end{align*} 
%
where for all $a \in \R$, $\sign(a) \cdot \infty = +\infty$ if $a > 0$, $-\infty$ otherwise. %, $1 \cdot \infty = +\infty$, and $-1 \cdot \infty = -\infty$.

We note that the standard STL robustness $\rho$ as defined in~\cite{DBLP:conf/formats/DonzeM10} can be recovered by letting $\rho(\f,w,t) = \rho_\esses^\emptyset(\f,w,t)$.
The notion of robustness that we define instead measures the robustness only on the subset of variables $\exes$, relative to some variables $\wyes$.
Variables in $\exes$ are measured, and their robustness is given by the terms they appear in; variables in $\wyes$ are considered fixed and their robustness is taken to be infinite; variables neither in $\exes$ nor in $\wyes$ are considered to take arbitrary values, and their robustness is zero.

\paragraph{Output Robustness and Input Vacuity}

We now specialize the notion of relative robustness to the context of input and output signals.
Let $(\exes, \wyes, \f)$ be an IA-STL specification. 
%
\begin{itemize}
\item We call {\em output robustness}, denoted $\mu$, the $\wyes$-robustness relative to $\esses\backslash\wyes$. By definition
$\mu(\f, w, t) \equiv \rho_\wyes^{\esses\backslash\wyes}(\f, w, t)$.
\item We call {\em input vacuity}, denoted $\nu$, the $\exes$-robustness relative to $\emptyset$. By definition $\nu(\f, w, t) \equiv \rho_\exes^{\emptyset}(\f, w, t)$. 
\end{itemize}
%
\begin{table}[H]
\caption{Possible combinations of output robustness and input vacuity values, where $k \in \R_{\ge 0}$, and their meaning.}
\begin{tabular}{ccc}
\toprule
$\mu(\f,w)$ & $\nu(\f,w)$ & Interpretation\\
\midrule
%$+\infty$ & $+\infty$ & tautology \\ 
$+\infty$ & $+k$      & vacuously true \\
$+k$      & $0$       & nonvacuously true \\
$-k$      & $0$       & nonvacuously false \\ 
$-\infty$ & $-k$      & vacuously false \\
%$-\infty$ & $-\infty$ & antilogy \\ 
\bottomrule
\end{tabular}
\label{tab:combination}
\end{table}
%

The output robustness represents the robustness of the specification relative to the trace, measured at the output.  
When positive (negative), it indicates by how much the output can be changed without falsifying (satisfying) 
the formula for the given input. When infinity (negative infinity), the output robustness indicates that $\f$ is vacuously satisfied (falsified) by the given input.

The input vacuity measure represents the level of vacuity of $\f$ with respect to the given input. 
When positive (negative) it indicates by how much the input can be changed without falsifying (satisfying) the formula, regardless of the output. 
When equal to $0$, the input vacuity indicates that the formula is non-vacuously true or false, based on trace $w$.

Table~\ref{tab:combination} summarizes the meaning of possible combinations of input vacuity and output robustness.\footnote{We remark that the meaning of $\mu(\f,w)=\nu(\f,w)=0$ is ambiguous, since it can be interpreted as $w$ satisfying or falsifying $\f$. This is related to the fact that in general the satisfaction/violation boundary may feature both satisfying and falsifying traces, so that borderline traces cannot be classified. We omit from the table the cases $\mu(\f,w) = \nu(\f,w) = \pm\infty$ as they can only happen when measuring robustness with formulas that are obvious tautologies and contradictions built using subformula $\top$, and are consequently of no practical interest.}

\newpage
\section*{Original TOC}
\begin{itemize}
    \item Define function under test and ODD
    \item[] (Sensors needed, simulator)
    \item Define Abstract Scenarios
    \begin{itemize}
        \item Describe scenario languages (OS, Scenic, Foretify) - give examples
        \item NHTSA pre-crash typology
    \end{itemize}
    \item From abstract to concrete scenarios
    \begin{itemize}
        \item Mention possible variables that are sampled
        \begin{itemize}
            \item Road Geometry
            \item Weather (Time of day, fog, rain, etc)
            \item Actor Init
            \item[] Actor Behavior Parameters
            \item[] Actor vehicle type/color/etc
            \item Ego Init conditions
        \end{itemize}
        \item Implicit vs Explicit variables
    \end{itemize}
    \item Specifications for use case and monitors
    \begin{itemize}
        \item  Multiple Types of Specifications (Safety, Comfort, Legal,..)
        \item List of specifications used and explanations
        \item[] Caveats for spec monitoring (``ahead of" , etc.)
        \item Scenario trace plots of spec robustness
    \end{itemize}
    \item Sampling scenarios
    \begin{itemize}
        \item Halton Sequences, CE, GLIS (explanation of each, and benefits)
        \item Reduction of search space
    \end{itemize}
    \item Assume $\rightarrow$ Guarantee examples
    \begin{itemize}
        \item Plots where other actors did not fulfil assumptions
        \item Composition of requirements
    \end{itemize}
    \item Sensitivity Analysis
    \begin{itemize}
        \item Variable reduction
        \item Plots (projection vs subspace)
    \end{itemize}
\end{itemize}
